One Layer's Trash is Another Layer's Treasure: Adaptive Layer-wise Visual Token Selection in LVLMs

Large Vision-Language Models (LVLMs) have achieved remarkable success across diverse multimodal tasks, yet their practical deployment remains constrained by the computational burden arising from lengthy visual tokens. While visual token pruning has emerged as a promising solution, existing methods suffer from a fundamental limitation: once tokens are pruned at a specific layer, they become inaccessible to all subsequent layers, leading to premature information loss that can compromise model performance. Through empirical studies, we observe that different layers exhibit distinct visual region focus, indicating a varying optimal token subset across layers. Motivated by this insight, we propose Adaptive Layer-wise Visual Token Selection (ALVTS), a novel framework that breaks away from the conventional static token pruning paradigm. ALVTS incorporates a lightweight token selector to identify and route important tokens for further processing, while allowing less important tokens to skip the layer, thus minimizing computational redundancy. These two streams of tokens are seamlessly reintegrated before being fed into subsequent layers, facilitating adaptive compression across the entire model. Grounded in our importance consistency constrained low-rank approximation, the proposed token selection module closely emulates the full attention mechanism, effectively capturing its essential patterns without requiring model retraining. Extensive experiments on LLaVA-1.5, LLaVA-NeXT, and Qwen2.5-VL validate the effectiveness of our method. With an 89% token compression ratio, ALVTS retains 96.7% of the original model's accuracy, achieving a superior efficiency-accuracy trade-off for LVLM inference.

==> sec/X_suppl_crversion.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
\appendix  % 自行添加

\section{Benchmark Details}
\label{sec:benchmark details}
\begin{itemize}
\item \textbf{AI2D}~\cite{kembhavi2016diagram} focuses on diagram interpretation and reasoning, comprising over 5,000 grade school science diagrams with comprehensive annotations. Each diagram is associated with multiple-choice questions, totaling more than 15,000 questions across the dataset. This benchmark is specifically designed to evaluate models' ability to understand complex visual structures, parse spatial relationships, and perform domain-specific semantic reasoning about scientific concepts depicted in diagrams.

\item \textbf{POPE}~\cite{li2023evaluating} assesses object hallucination in large vision-language models by formulating evaluation as a binary classification task using simple yes-or-no questions. Built on the MS COCO validation set, we evaluate on 500 randomly selected images with 6 questions per image, totaling 3,000 question-answer pairs. Three sampling strategies are employed: random, popular, and adversarial. The adversarial strategy is particularly critical as it targets objects that frequently co-occur with the ground truth but are not present in the image, thereby rigorously testing the model's tendency to hallucinate based on contextual priors rather than visual evidence. Performance is measured using accuracy, precision, recall, and F1 score.

\item \textbf{TextVQA}~\cite{singh2019towards} addresses visual question answering requiring reading and reasoning about text in images, containing 45,336 questions on 28,408 images sourced from the Open Images dataset. Each question is annotated with 10 human-provided answers, with the dataset split into 34,602 training, 5,000 validation, and 5,734 test questions. Evaluation follows the standard protocol where the predicted answer is compared against 10 human annotations. An answer is considered correct if it matches at least 3 out of 10 human responses. The benchmark tests models' ability to detect, recognize, and reason about textual content embedded within natural scene images. 

\item \textbf{OKVQA}~\cite{marino2019ok} features 14,055 questions where image content alone is insufficient for answering, requiring external knowledge resources. Questions are collected on COCO images, with 9,009 training and 5,046 test samples, each accompanied by 10 answer annotations. The dataset spans 10 knowledge categories including science, history, sports, and geography. We follow the standard evaluation protocol using the VQA accuracy metric, comparing predicted answers against human annotations.

\item \textbf{VizWiz}~\cite{gurari2018vizwiz} is a goal-oriented VQA dataset comprising over 31,000 visual questions from blind users who captured images via mobile phones and recorded spoken queries. Each image is annotated with 10 crowdsourced answers. The dataset presents unique challenges including poor image quality (blur, lighting issues, obstructed views) and conversational question styles. We evaluate on the test split using the standard VQA accuracy metric.

\item \textbf{COCO Caption}~\cite{lin2014microsoft} is built upon the MS COCO dataset, which contains 328,000 images depicting complex everyday scenes with common objects in natural contexts. The dataset comprises 91 object categories and 2.5 million labeled instances. Each image is paired with five human-generated descriptive captions collected via crowdsourcing. Following standard practice, we report CIDEr as the primary captioning metric for performance assessment.

\item \textbf{NoCaps}~\cite{agrawal2019nocaps} is a novel object captioning benchmark consisting of 15,100 images from Open Images with 166,100 human-generated captions. Each image contains 10 reference captions plus one human baseline caption. Test images are divided into in-domain, near-domain, and out-of-domain subsets based on object category overlap with COCO. Specifically, in-domain images contain only objects belonging to COCO classes; near-domain images include a mix of both COCO and novel classes; while out-of-domain images consist exclusively of novel classes. We evaluate on all three splits using the CIDEr metric.

\item \textbf{RealWorldQA} is a real-world visual understanding benchmark containing 765 images captured from vehicles and diverse real-world settings. Each image is paired with a question requiring visual reasoning and a verifiable answer. Questions span object recognition, spatial relationships, directional understanding, and scene comprehension. We report accuracy on the full test set.
\end{itemize}


% ------------------------------
\section{Implementation Details}
Experiments with LLaVA-1.5-7B~\cite{liu2024improved}, LLaVA-NeXT-7B~\cite{liu2024llavanext}, and Qwen2.5-VL-3B-Instruct~\cite{bai2025qwen2} models are conducted on a single NVIDIA GeForce RTX 4090 GPU. Experiments with the LLaVA-1.5-13B model are conducted on a single NVIDIA A100-40G GPU. The implementation is carried out in Python
3.10, utilizing PyTorch 2.1.2 and CUDA 12.2. The inference follows the evaluation settings of the LMMs-Eval framework~\cite{zhang2025lmms}.


% ------------------------------
\section{LLaVA-1.5-13B Detailed Results}
% 表格
\input{tables/crversion_appendix_13b}
\input{tables/crversion_appendix_rank_choice}
\cref{tab:crversion_appendix_13b} presents the detailed per-benchmark performance of LLaVA-1.5-13B under different token reduction ratios. At a 67\% reduction ratio, ALVTS attains 99.86\% average performance, outperforming all competing methods. Notably, ALVTS maintains robust performance even at an 89\% reduction ratio, achieving 96.63\% versus 91.20\% for FastV~\cite{chen2024image}. The method demonstrates particular strength on challenging benchmarks like COCO Caption and NoCaps, validating its effectiveness in preserving critical visual information under aggressive compression.


% ------------------------------
\section{Ablation Study about Token Selector Rank}
To determine the optimal rank for the token selector, we evaluate ALVTS with different rank settings, as shown in \cref{tab:crversion_appendix_rank_choice}. We observe that increasing the rank from 32 to 256 brings notable performance improvements across all benchmarks, lifting the average performance from 90.67\% to 94.72\%. However, further increasing the rank from 256 to 384 yields only marginal gains (94.72\% to 94.95\%), while the parameter overhead per decoder layer increases from 2.07\% to 3.11\%. Therefore, we select a rank of 256 for LLaVA-1.5-7B, as it provides an optimal balance between model performance and parameter efficiency.

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

%-------------------------------------------------------------------------
\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

==> tables_rebuttal/R1Q1_rank_selection.tex <==
\begin{table}[t]
    \caption{Ablation study on token selector rank in LLaVA-1.5-7B under 89\% token compression ratio. Avg. denotes the average performance across 4 benchmarks relative to the original model, and Overhead indicates the parameter overhead per decoder layer.}
    \label{tab:rank_selection}
    \vspace{-5pt}  % 减小captain与表格主体的间距

    % 将表格内所有字体缩小
    \footnotesize
    % 稍微减小列间距，为内容和竖线腾出空间
    \setlength{\tabcolsep}{3pt}
    % 减小booktabs规则线与内容的间距
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}

    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}} ccccccc}
    \toprule
    \textbf{Rank} & \textbf{POPE} & \textbf{OKVQA} & \textbf{COCO} & \textbf{NoCaps} & \textbf{Avg.} & \textbf{Overhead} \\
    \midrule
    32 & 79.10 & 47.87 & 101.51 & 94.08 & 90.67\% & 0.26\% \\
    64 & 81.68 & 48.33 & 105.73 & 95.50 & 92.93\% & 0.52\% \\
    128 & 83.38 & 48.57 & 106.33 & 96.17 & 93.83\% & 1.04\% \\
    256 & 83.87 & 49.66 & 105.89 & 97.60 & 94.72\% & 2.07\% \\
    384 & 84.07 & 49.77 & 106.64 & 97.38 & 94.95\% & 3.11\% \\
    512 & 84.34 & 50.13 & 106.46 & 97.80 & 95.26\% & 4.15\% \\ 
    \bottomrule
    \end{tabular*}
    \vspace{-3pt}
\end{table}
% \linespread{0.9}\selectfont

==> tables_rebuttal/R1Q2_latency_breakdown.tex <==
\begin{table}[t]
    \caption{Latency breakdown (ms) of LLaVA-1.5-7B on the POPE dataset with 89\% token compression ratio.}
    \label{tab:latency_breakdown}
    \vspace{-5pt}  % 减小captain与表格主体的间距

    % 将表格内所有字体缩小
    \footnotesize
    % 稍微减小列间距，为内容和竖线腾出空间
    \setlength{\tabcolsep}{3pt}
    % 减小booktabs规则线与内容的间距
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}

    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccc@{}}
    \toprule
    \textbf{Method} & \textbf{Selector} & \textbf{Attention} & \textbf{FFN} & \textbf{Total} \\
    \midrule
    \multicolumn{5}{c}{batch size = 1} \\
    \midrule
    Vanilla & - & 74.8 \scriptsize{(all tokens)} & 90.9 \scriptsize{(all tokens)} & 165.7 \\
    ALVTS & 38.6 \scriptsize{(all tokens)} & 35.4 \scriptsize{(11\% tokens)} & 29.5 \scriptsize{(11\% tokens)} & 103.5 \\
    \midrule
    \multicolumn{5}{c}{batch size = 4} \\
    \midrule
    Vanilla & - & 278.2 \scriptsize{(all tokens)} & 344.7 \scriptsize{(all tokens)} & 622.9 \\
    ALVTS & 112.5 \scriptsize{(all tokens)} & 85.8 \scriptsize{(11\% tokens)} & 105.7 \scriptsize{(11\% tokens)} & 304.0 \\
    \bottomrule
    \end{tabular*}
    \vspace{-3pt}
\end{table}


==> tables_rebuttal/R2Q1_calibration_source.tex <==
\begin{table}[t]
    % 减小caption行间距
    \caption{Ablation study on calibration data sources under different token compression ratios. Avg. refers to the average performance across 8 benchmarks.}
    \label{tab:calibration_source}
    \vspace{-5pt}  % 减小captain与表格主体的间距

    % 将表格内所有字体缩小
    \footnotesize
    % 稍微减小列间距，为内容和竖线腾出空间
    \setlength{\tabcolsep}{2pt}
    % 减小booktabs规则线与内容的间距
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}

    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccc@{}}
    \toprule
    \textbf{Calibration Source} & \textbf{Avg. (\text{\footnotesize $\downarrow$ 67\%})} & \textbf{Avg. (\text{\footnotesize $\downarrow$ 78\%})} & \textbf{Avg. (\text{\footnotesize $\downarrow$ 89\%})} \\
    \midrule
    LLaVA-655k {\footnotesize\textit{(Ours)}} & 99.60\% & 98.77\% & 96.73\% \\
    COCO {\footnotesize\textit{(Natural Images)}} & 99.37\% & 99.18\% & 97.03\% \\
    VQA$^{\text{Text}}$ {\footnotesize\textit{(Text-Rich)}} & 99.70\% & 99.36\% & 96.68\% \\
    AI2D {\footnotesize\textit{(Diagrams)}} & 99.51\% & 99.01\% & 96.96\% \\
    \bottomrule
    \end{tabular*}
    \vspace{-3pt}
\end{table}



==> tables_rebuttal/R3Q3_selector_interval.tex <==
\begin{table}[t]
    \caption{Ablation study on token selector placement frequency. We report the average performance across 8 benchmarks under 89\% token compression ratio.}
    \label{tab:selector_interval}
    \vspace{-5pt}  % 减小captain与表格主体的间距

    % 将表格内所有字体缩小
    \footnotesize
    % 稍微减小列间距，为内容和竖线腾出空间
    % \setlength{\tabcolsep}{3pt}
    % 减小booktabs规则线与内容的间距
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}

    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}ccc@{}}
    \toprule
    \textbf{Every Layer} & \textbf{Every 2 Layers} & \textbf{Every 3 Layers} \\
    \midrule
    96.73\% & 96.07\% & 85.35\% \\
    \bottomrule
    \end{tabular*}
    \vspace{-10pt}
\end{table}

